On the Security Bootstrapping in Named Data Networking

By requiring all data packets been cryptographically authenticatable, the Named Data Networking (NDN) architecture design provides a basic building block for secured networking. This basic NDN function requires that all entities in an NDN network go through a security bootstrapping process to obtain the initial security credentials. Recent years have witnessed a number of proposed solutions for NDN security bootstrapping protocols. Built upon the existing results, in this paper we take the next step to develop a systematic model of security bootstrapping: Trust-domain Entity Bootstrapping (TEB). This model is based on the emerging concept of trust domain and describes the steps and their dependencies in the bootstrapping process. We evaluate the expressiveness and sufficiency of this model by using it to describe several current bootstrapping protocols.

==> Makefile <==
PRJ = ndn-bootstrap

ifdef S
EXTRA = -synctex=1
endif

all : ${PRJ}.pdf

${PRJ}.pdf : sections/*.tex *.tex *.bib
	pdflatex ${EXTRA} ${PRJ} && \
		(ls ${PRJ}.aux | xargs -n 1 bibtex) && \
		pdflatex ${EXTRA} ${PRJ} && pdflatex ${EXTRA} ${PRJ}

view : ${PRJ}.pdf
	open ${PRJ}.pdf &

clean:
	/bin/rm -f ${PRJ}.pdf *.toc *.aux *.bbl *.blg *.log *~* *.bak *.out *synctex.gz

distclean: clean
	/bin/rm -f ${PRJ}.pdf



==> sections/tib.tex <==
\section{Trust Information Base}
\label{sec:tib}
\ty{somewhere, we need paragrahs to talk about the security assumptions for both TIB and validated key cache}
In this section, we show how Trust Information Base (TIB) manages trust relations for entities.
TIB is a functional module for entities inside trust zone.
It has its own Keychain and provides library calls for entities to perform security bootstrapping.
During bootstrapping, TIB loads trust anchor and trust schema and installs the certified identities\ty{need to explain why can have multiple} into Keychain. 
After that initialization step, a TIB instance is enabled to secure data communications in application runtime.

\subsection{Automated Security Workflow}
\label{sec:tib-workflow}
\ty{I felt I didn't explain NAC enough, meybe this section needs expansion}
NDN security models provide the foundation for automating security workflows and make then transparent to application developers.
TIB embeds name-based security models and realizes the security workflow for Data production and consumption.
In this section, we demonstrate TIB security workflow in Figure~\ref{fig:bootstrap-tib}.
We assume each TIB instance was initilized from entity security bootstrapping.
The trust zone controller also serves as an access manager for Named-based Access Control (NAC)~\cite{zhang2018nac}.
Before bootstrapping the producer and consumer entitiy, trust zone controller pre-generates KDK and KEK for each name prefix based on the access control policy.

\begin{figure}[ht]
    \centering
	\includegraphics[width=0.47\textwidth]{figs/bootstrap-tib}
	\caption{TIB Security Workflow\ty{the figure needs revision}}
	\label{fig:bootstrap-tib}
\end{figure}

\mypara{\textit{Produce(name, content)$\rightarrow$(AppData, CKData)}}
In order to secure data production, the producer entity calls the TIB library function \textbf{\textit{Produce}} with data name and content.
TIB does the following steps to secure the data production.
Firstly, TIB follows the NAC model to generate Content Encryption Key (CK) and uses CK to encrypt the content.
In order to encrypt CK, TIB expresses Interest to fetch corresponding Key Encryption Key (KEK) for the data prefix.
Secondly, TIB uses trust schema to match a data signing certificate from its KeyChain.
If there is a certificate match, TIB uses Keychain to sign the encrypted content.
It also generates CK Data with the trust schema allowed signing certificate.
The CK Data encapsulates encrypted CK for data consumers to fetch.
Finally, TIB returns the signed Application Data packet with the corresponding CK Data.
The producer entity further passes the secured application Data packet to the transport layer (\eg SVS~\cite{}) or the forwarder.
It also serves the corresponding CK Data through either through the transport function or direct prefix registration. 

\mypara{\textit{Consume(AppData)$\rightarrow$(name, content)}}
On the data consumption side, the consumer entity calls the TIB library function \textbf{\textit{Consume}} with the received Data packet.
TIB will first look up the Data's KeyLocator and recursively fetch the signing certificate until reaching a self-signed certificate.
Then it begins validates the certificate chain with the trust anchor and trust schema.
Upon successful chain verification, TIB parses the CK name from the Data content and uses the NAC convention to construct the corresponding KDK name.
Then TIB expresses Interest to fetch the Key Decryption Key (KDK) Data and CK Data from the producer entity.
After validating KDK and CK Data, it uses KDK to decrypt CK from the CK Data and futher use CK to decrypt the original Data content.
As the last step, TIB returns name and content to the consumer entity.

\subsection{Optimizing Certificate and Key Validation}
\ty{need to mention security assumptions and it first appeared in Yingdi's paper. Also I don't think we need a such long section.}
As shown in Figure~\ref{fig:bootstrap-tib}, consuming a application Data packet requires TIB retrieving and validating several certificate and key Data packets in a row.
In a trust zone with long certificate chain, such Interest-Data exchanges and cryptographic operations add noticeable latency to the application data communications.
NDN's in-network caching mechanism (\ie Content Store) can mitigate the problem, but cannot become a reliable solution for two reasons. 
First, the consumer entity has no control over the forwarder caching policy, therefore the certificate and key availability from the forwarder Content Store is unpredictable.
Second, Content Store in the network layer is agnostic to application trust zones.
Therefore, TIB needs to validate each Data returned by the Content Store, even the same Data has been validated in the last Data consumption workflow.

A consumer-controlled \textit{validated key cache} can solve this problem by caching TIB validated certificates and keys into a consumer-controlled storage space.
The consumer entity can configure a validated key cache to an initialized TIB.
As a result, when TIB needs a certificate, KDK Data, or CK Data in security workflow, it looks up the Data in validated key cache.
TIB only expresses Interest and validates the retrieved certificate chain on a cache miss.
When TIB successfully validates an certificate and key Data, it writes to the validated key cache for future use.
Since the consumer entity has full control of the validated key cache, we assume it runs the validated key cache with the optimal cache policy of its application.
\begin{figure}[ht]
    \centering
	\includegraphics[width=0.48\textwidth]{figs/bootstrap-tib-cache}
	\caption{Validated Key Cache helps data validation}
	\label{fig:bootstrap-tib-cache}
\end{figure}

Figure~\ref{fig:bootstrap-tib-cache} illustrates how validated key cache reduce the average latency of validating long certificate chain.
In this example, the producer certificate is on the fifth level of the certificate chain.
We assume the validated key cache is empty before TIB starts validating AppData 1. 
In order to validate the AppData 1, TIB needs to fetch all five certificates on the chain and start validation from the trust anchor.
Each time TIB looks up the certificate name in validated key cache and get a cache miss, thereby it lookups the KeyLocator and fetches the upstream signing certificate until reaching the trust anchor.
Then it starts certificate chain validation from the trust anchor, and writes each validated certificate to cache.
When later TIB validates AppData 2 signed by the same producer certificate, it finds producer certificate from the cache and directly using the cache result to validate AppData 2.
Although this example shows validated key cache has great potential to reduce the verification latency, the actual performance improvement is up to deployment specific cache capacity and policies specified by the consumer entity.

==> sections/toolset.tex <==
\section{\sysname\ Design}
As stated, modeling security bootstrapping (Section~\ref{sec:bootstrap}) not only helps us better understand the existing solutions but also blueprints future protocol designs.
\ty{need to say sth similar in section~\ref{sec:bootstrap}}
TIB (Section~\ref{sec:tib}) as a functional module provides library calls for NDN entities to perform security bootstrapping, and automates security workflow utilizing naming conventions.
\ty{somewhere in section~\ref{sec:tib} we need to explain it is the naming convention enpowers TIB.}
We realizes the two aforementioned ideas and provides security support for trust zone controller and entities in a toolset named \sysname.
In this section, we first use an example to provide an overview of \sysname\ design, then introduce individual components from an developer perspective.

\subsection{An Overview}
\label{sec:toolset-overview}
Figure~\ref{fig:ntrust-overview} visualizes the high-level overview of a \sysname\ enpowered trust zone.
Let us assume the NDNFit~\cite{zhang2016sharing} developer wants to start a trust zone \name{/ndnfit} and invite Alice and Bob as users.
Therefore, the developer first self signs the certificate for \name{/ndnfit} as trust anchor and determines the entity naming conventions (Section~\ref{sec:toolset-enew-name}). 
Then the developer (i) completes the namespace and trust schema design based on pre-generated schema templates (Section~\ref{sec:toolset-schema-templates}); (ii) specifies name-based access control policies and generate corresponding KEKs and KDKs (Section~\ref{sec:toolset-acp}); (iii) realizes the abstract bootstrapping functions.
In order to update trust schema after entity bootstrapping, the NDNFit trust zone controller is enabled to publish entity-specific trust schema as Data packets (Section~\ref{sec:toolset-schema-publisher}).
In development, one further optimizes certificate availability (Section~\ref{sec:toolset-cert-avail}) by providing redundancies.
As the last step, the developer packages the implementation and distributes to the users.

\begin{figure}[ht]
    \centering
	\includegraphics[width=0.47\textwidth]{figs/ntrust-overview}
	\caption{A high-level overview of a \sysname\ enpowered trust zone}
	\label{fig:ntrust-overview}
\end{figure}

\subsection{Entity Name Assignment}
\label{sec:toolset-enew-name}
An entity name must be \textit{unique} and \textit{semantically meaningful}, and both can be achieved through making use of existing authenticated identifiers.
Trust zone controller bootstraps each entity based on their existing trust relations (see Section~\ref{sec:bootstrap-enewauth}).
In some scenarios, new entity's authentication identifier (\eg email, DNS name) have semantically encoded its existing trust relations.
As a result, the controller can name new entity by converting its semantically meaningful and authenticated identifier into an NDN name.

We perform the \textit{semantic conversion} via the VerSec language\footnote{Although VerSec was originally purposed for trust schema, we found its syntax is also expressive in other areas.}.
For example, Alice is identified by her email address \name{alice@example.com}, whose semantics consists of domain name and user name.
Note that in order to possess this email, example.com must authenticate Alice and ensures the user name uniqueness inside the domain.
Let us assume the NDNFit controller uses the second level domain and user name for naming.
Specifically, it converts email address into an NDN name \name{/<user>/<sld>/<tld>}\footnote{<> indicates a wildcard name component}, and specifies the entity naming convention \name{/ndnfit/<sld>/<user>}.
The developer can express this name mapping in VerSec:
\VerSec
\begin{lstlisting}
#email: /user/sld/tld
#entityName: /"ndnfit"/sld/user <= #email
\end{lstlisting}
The above code snippets map the Alice's email address into NDN name \name{/ndnfit/example/alice}.
In order to reduce the attack surface, \sysname\ enforces the unique mapping between authentication identifier and entity name.
Alice's email address cannot be used to authenticate multiple entities, but rather is strictly binded to the named entity \name{/ndnfit/example/alice}.

The developer can rely on semantic conversion for semantically meaningful identifiers.
However in cases where authentication identifiers do not have sufficient semantics for naming (\eg SSH and GPG\cite{} keys), the controller needs other information source for naming.
Assuming Bob is authenticated through his SSH key named \name{bob@laptop}, the developers specifies the semantic conversion rules as below:
\VerSec
\begin{lstlisting}
#ssh: /user/host
#entityName: /"ndnfit"/host/user <= #ssh
\end{lstlisting}
In this case
The semantic conversion produces \name{/ndnfit/laptop/bob}, but the host name \name{laptop} is not unique.
As a result, the controller attaches the first few bytes of public key hash after it thus uniquely names Bob as \name{/ndnfit/laptop/bob/0d1d11c}.

\subsection{Rule and Schema Templates}
\label{sec:toolset-schema-templates}
\ty{this should go into motivation, but our motivation is already embedded in the introduction}
% A key observation that motivates the schema template design is that current applications incline to validate packets permissively.
% Because lacking useful tools, except the recently proposed DCT, to legitimately sign packets based on trust schema, the developers tend to have loose signing restrictions for convienence.
% A typical example of loose restrictions is only validating the packet name under the namespace of packet signer.
A key observation that motivates the rule and schema templates design is that trust schemas are structured.
Figure~\ref{fig:versec-example} shows the trust schema of the python-ndn consumer example~\cite{}.
The trust schema starts from defining the certificate suffix "\#KEY" and global keywords "\#site".
Then the schema further derives the signing restrictions for application Data "\#article" and step-by-step specifies its upstream signers until reaching the trust anchor "\#root", which is defined in the last line.
If the adminstrators uses NDNCERT to issue certificates for authors, one needs rules as Figure~\ref{fig:ndncert-versec} to validate NDNCERT Data.
% Note that the above rules do not restrict the issuer of \#admin" signing certificate.
% Note that in the above process, the developer needs to handcrafts trust schema.
% As a result, the developer has to either learn the NDNCERT packet format or use permissive validation rules instead.

\begin{figure}[!t]
\VerSec
\begin{lstlisting}
#KEY: "KEY"/_/_/_
#site: "lvs-test"
#article: #site/"article"/author/post/_version & {_version: $eq_type("v=0")} <= #author
#author: #site/"author"/author/"KEY"/_/admin/_ <= #admin
#admin: #site/"admin"/admin/#KEY <= #root
#root: #site/#KEY
\end{lstlisting}
\caption{An exmaple of VerSec based trust schema}
\label{fig:versec-example}
\end{figure}

\begin{figure}[!t]
\VerSec
\begin{lstlisting}
#newResponse: #site/"CA"/"NEW"/_ <= #admin
#challengeResponse: #site/"CA"/"CHALLENGE"/_/_ <= #admin
\end{lstlisting}
\caption{An exmaple of VerSec based NDNCERT Data validation rules}
\label{fig:ndncert-versec}
\end{figure}

We designed rules templates to provide templates for commonly used naming conventions, application protocols, and trust zone operations (\eg deriving certificate chain).
Developers pass name components to templates as parameters so that they do not need to write the same validation rules for different applications.
As Figure~\ref{fig:example-template} shows, the developers can call \sysname\ functions to generate individual validation rules and chain all validation rules to to realize the same trust schema.

\begin{figure}[!t]
\VerSec
\begin{lstlisting}
zone = define_zone("lvs-test")
root = define_anchor(zone)
admin = derive_cert(zone, "/"admin"/admin", from = root)
author = derive_cert(zone, "/"author"/author", from = admin)
article = define_versioned_data(zone, "/"article"/author/post", signed_by = author)
ndncert_proto = define_ndncert(zone, issuer = admin)
schema = zone + root + admin + author + article + ndncert_proto
\end{lstlisting}
\caption{Developing trust schema with \sysname\ rule templates}
\label{fig:example-template}
\end{figure}

Based on rule templates, we further designed schema templates for a minimal trust zone.
A minimal trust zone contains a trust anchor, and entities whose names have one name component suffix after the zone name and are certified by the trust anchor.
For example, the NDNFit developer as mentioned in Section~\ref{sec:toolset-overview} can define a minimal trust zone of \name{/ndnfit} by calling \sysname\ function:
\VerSec
\begin{lstlisting}
schema = define_minimal_trust_zone("ndnfit")
\end{lstlisting}
The developers can modify or extend this "minimal trust zone" schema template to accommodate their applications.
As a start point, \sysname\ provides schema templates for sample applications such as blog website and health data sharing.

Rule and schema templates simplify the trust schema development by 
(i) hiding low-level and protocol specific naming conventions from the developers so that they can focus on the application namespace design; 
(ii) providing abstractions to design trust schema based on application scenarios\ty{put details in appendix?}.
(iii) enabling developers to program trust schema in the same language as their application development (\eg Python, C++).


\subsection{Access Control Policies}
\label{sec:toolset-acp}
\ty{we didn't have a concrete design, but we need to do some hand waving here to show trust zone operator specifies NAC policies}
\subsection{Bootstrapping Support}
% \subsection{Name Based Access Control over Entity Roles}
% \ty{performing NAC over role attached entitiy names}
\subsection{Schema Publisher and Fetcher}
\label{sec:toolset-schema-publisher}
\subsection{Certificate Availabilty}
\label{sec:toolset-cert-avail}
\ty{validated key cache, register identity prefix for own certificates}
